Automatic Generation of Hierarchical Contracts for Resilience in Cyber-Physical Systems

With the growing scale of Cyber-Physical Systems (CPSs), it is challenging to maintain their stability under all operating conditions. How to reduce the downtime and locate the failures becomes a core issue in system design. In this paper, we employ a hierarchical contract-based resilience framework to guarantee the stability of CPS. In this framework, we use Assume Guarantee (A-G) contracts to monitor the non-functional properties of individual components (e.g., power and latency), and hierarchically compose such contracts to deduce information about faults at the system level. The hierarchical contracts enable rapid fault detection in large-scale CPS. However, due to the vast number of components in CPS, manually designing numerous contracts and the hierarchy becomes challenging. To address this issue, we propose a technique to automatically decompose a root contract into multiple lower-level contracts depending on I/O dependencies between components. We then formulate a multi-objective optimization problem to search the optimal parameters of each lower-level contract. This enables automatic contract refinement taking into consideration the communication overhead between components. Finally, we use a case study from the manufacturing domain to experimentally demonstrate the benefits of the proposed framework.

==> authors.tex <==

%\author{Zhiheng Xu$^1$, Daniel Jun Xian Ng$^1$, Arvind Easwaran$^1$, and Sidharta Andalam$^2$}
%\affiliation{\vspace{1mm}
%  \institution{$^1$Nanyang Technological University and
%  $^2$Delta Electronics, 50 Nanyang Avenue, Singapore, 639798}
%  Email: $^1$\{zhiheng.xu, danielngjj, arvinde\}@ntu.edu.sg and
%  $^2$sidharta.andalam@deltaww.com
%}

\author{Zhiheng Xu}
\affiliation{Nanyang Technological University, \\
50 Nanyang Avenue, Singapore}
\email{zhiheng.xu@ntu.edu.sg}

\author{Daniel Jun Xian Ng}
\affiliation{Nanyang Technological University, \\
50 Nanyang Avenue, Singapore}
\email{danielngjj@ntu.edu.sg}

\author{Arvind Easwaran}
\affiliation{Nanyang Technological University, \\
50 Nanyang Avenue, Singapore}
\email{arvinde@ntu.edu.sg}

\author{Sidharta Andalam}
\affiliation{Delta Electronics, \\
50 Nanyang Avenue, Singapore}
\email{sidharta.andalam@deltaww.com}

% The default list of authors is too long for headers.
\renewcommand{\shortauthors}{Z. Xu and D. J. X. Ng et al.}
